SQFT: Low-cost Model Adaptation in Low-precision Sparse Foundation Models

Large pre-trained models (LPMs), such as large language models, have become ubiquitous and are employed in many applications. These models are often adapted to a desired domain or downstream task through a fine-tuning stage. This paper proposes SQFT, an end-to-end solution for low-precision sparse parameter-efficient fine-tuning of LPMs, allowing for effective model manipulation in resource-constrained environments. Additionally, an innovative strategy enables the merging of sparse weights with low-rank adapters without losing sparsity and accuracy, overcoming the limitations of previous approaches. SQFT also addresses the challenge of having quantized weights and adapters with different numerical precisions, enabling merging in the desired numerical format without sacrificing accuracy. Multiple adaptation scenarios, models, and comprehensive sparsity levels demonstrate the effectiveness of SQFT. Models and code are available at https://github.com/IntelLabs/Hardware-Aware-Automated-Machine-Learning.

==> content/2_related_w.tex <==
\section{Related Work}
\label{sec:related}

Generative pre-trained models often based on the Transformer architecture \cite{Transformer_NIPS2017} require the application of compression techniques to reduce their significant computational cost and to address challenges, e.g., related to memory bandwidth. Classic compression techniques like pruning and quantization have been adapted to the age of LPMs, removing inefficiencies that cannot be tolerated when dealing with billions of parameters. We discuss them in more detail next. 

\paragraph{Pruning} Inducing sparsity, either by zeroing out weights or activations or removing network elements, can improve the efficiency of LPMs during inference, provided that they are executed on a runtime that can exploit sparse patterns. Pruning has a long history \cite{LeCunBrainDamage}, but with the advent of LPMs, traditional methods\cite{hoeflerSparsity21}, e.g., Magnitude Pruning \cite{HAGIWARA1994207}, have been replaced by new approaches that are suited for the challenges of these models. In particular, due to their large number of parameters. SparseGPT \cite{frantar-sparsegpt} proposes a one-shot pruning method for transformer-based models that trade minimal accuracy drop for increasing sparsity levels. The method approaches LPMs' pruning layer-wise with an efficient weight reconstruction algorithm that incrementally prunes the weight matrix elements. Wanda \cite{sun2023wanda} proposes a more straightforward approach that does not require weight updates, computing a score using the weight magnitude and the norm of input activations. This approach obtains better results than SparseGPT. Recently, BESA \cite{xu2024besa} improves over SparseGPT and Wanda by targeting individual transformer blocks and allocating sparsity per layer using a differentiable method. 
These approaches induce sparsity on pre-trained models and are evaluated on zero-shot benchmarks. Our end-to-end solution, \proj, focuses on further adapting the sparsified models to new tasks or datasets. 

\begin{figure*}[ht]
    \includegraphics[width=\textwidth]{figures/overview.pdf}
    \caption{\proj Overview. Several pipeline configurations can be activated to efficiently fine-tune large models while addressing several limitations of existing approaches.  
}\label{fig:overall_pipeline}    
\end{figure*}

\paragraph{Quantization} 
In the era of large pre-trained foundation/frontier models (LPMs), quantization approaches have evolved to address the challenges of scale and memory bandwidth. Due to the high cost of retraining these models to recover accuracy degradation, special consideration has to be taken when incorporating compression techniques, like quantization-aware training in foundation models. Post-training, one-shot quantization methods have prevailed, obtaining quantized versions of large models in hours. 
LLM.Int8() was among the first Int8 quantization procedures for large-scale transformer-based PLMs
\cite{dettmers2022LLMInt8}. Using vector-wise quantization and mixed-precision decomposition, LLM.Int8() demonstrated that it can effectively confront the outliers that emerge in activations, which makes traditional quantization methods fail in models with more than 6.7B parameters. In a contemporary work, after running thousands of experiments with various large pre-trained models, it was demonstrated that 4-bit parameters can reach optimal performance compared to other bit-precisions in the 3 to 16-bit range \cite{case4bit22}. 
ZeroQuant \cite{NEURIPS20ZeroQuant} quantizes GPT-3 models, obtaining a reduction in latency up to 4.16x by utilizing group-wise quantization for weights, token-wise quantization for activations, and layer-by-layer knowledge distillation. SmoothQuant \cite{xiao2023smoothquant} makes activations easier to quantize by smoothing them and compensating this operation with a transformation of the weights, resulting in improved results over ZeroQuant and LLM.Int8(). GPTQ is another good representative of one-shot quantization approaches designed especially for LPMs \cite{frantar-gptq}. GPTQ builds on the learnings from Optimal Brain Quantization (OBQ) \cite{frantar2022obc} and applies layer-wise quantization to the full-precision weights of a base LPM. We incorporate GPTQ as the default quantization method in \proj's pre-fine-tuning stage.

% \todo[inline]{
% GPTQ vs RTN in GPTQ paper - GPTQ is more stable and outperforms RTN. 

% GPTQ - Baseline used for PEQA 

% Round-to-nearest (RTN) - PEQA Used. 

% AutoGPTQ - https://github.com/AutoGPTQ/AutoGPTQ

% Mention limitations of PTQ 

% QuIP and QuIP\# 

% HQQ \cite{badri2023hqq}
% }

\paragraph{Parameter-efficient Fine-tuning (PEFT)} Due to their large number of parameters, it is too costly to fine-tune pre-trained large models. Updating all their weights to improve their performance in a downstream task might require devices with large memory capacity. PEFT techniques attempt to address this challenge by avoiding the update of all weights in the pre-trained model. For instance, low-rank (LoRA) adapters \cite{hu2022lora} use a fraction (often less than 1\%) of additional weights to adapt the model to a new task. LoRA adapters, $\boldsymbol{B}$ and $\boldsymbol{A}$, are utilized to reparameterize a linear projection, $\boldsymbol{Y} = \boldsymbol{WX}$, keeping the weights, $\boldsymbol{W}$, frozen and updating only the low-rank adapter matrices, $\boldsymbol{A}$ and $\boldsymbol{B}$, i.e., $\boldsymbol{Y} = \boldsymbol{WX} + \boldsymbol{BAX}$. 

Recently, Shears proposed Neural Low-rank Adapter Search \cite{shears} and demonstrated that LoRA adapters can be made elastic to allow for the application of weight-sharing schemes and keeping the original weights of the model frozen and compressed, e.g., inducing sparsity before the fine-tuning stage. However, a challenge that emerges is that merging the dense adapters with the sparse weights results in the overall loss of sparsity. LoRAPrune has attempted to address this challenge by using the weights and gradients of the LoRA adapters to remove elements in the model's weights  \cite{zhang2023loraprune}. In the approach discussed in this paper, \proj, we propose an alternative method for merging the dense adapters with a minimal drop in accuracy. The proposed solution is discussed next.   

